FeatGraph: A Flexible and Efficient Backend for Graph Neural Network Systems

Graph neural networks (GNNs) are gaining increasing popularity as a promising approach to machine learning on graphs. Unlike traditional graph workloads where each vertex/edge is associated with a scalar, GNNs attach a feature tensor to each vertex/edge. This additional feature dimension, along with consequently more complex vertex- and edge-wise computations, has enormous implications on locality and parallelism, which existing graph processing systems fail to exploit. This paper proposes FeatGraph to accelerate GNN workloads by co-optimizing graph traversal and feature dimension computation. FeatGraph provides a flexible programming interface to express diverse GNN models by composing coarse-grained sparse templates with fine-grained user-defined functions (UDFs) on each vertex/edge. FeatGraph incorporates optimizations for graph traversal into the sparse templates and allows users to specify optimizations for UDFs with a feature dimension schedule (FDS). FeatGraph speeds up end-to-end GNN training and inference by up to 32x on CPU and 7x on GPU.

==> figure_tex/fig_effect_hybrid_partitioning_gpu.tex <==
\begin{figure}[t]
\centering

\includegraphics[width=0.75\linewidth]{figure_raw/effect_hybrid_partitioning_gpu_spmm_rand_100K.pdf}

\caption{Effect of hybrid partitioning on the GPU performance of GCN conv. Tested on \texttt{rand-100K}.}
% \yida{Is training time per epoch? Is inference time per sample/batch? We should clarify this.}\reply{I added "time is for one epoch" in table 3}
\label{fig:effect-hybrid-partitioning-gpu-spmm}
%\vspace{-0.5em}
\end{figure}


==> figure_tex/fig_effect_tiling_cpu_spmm_reddit.tex <==
\begin{figure}
\centering

\includegraphics[width=0.75\linewidth]{figure_raw/effect_tiling_cpu_1_thread_spmm_reddit.pdf}

\caption{Effect of graph partitioning and feature dimension tiling on the CPU performance of GCN conv. Tested on \texttt{reddit}.}
\label{fig:effect-tiling-cpu-spmm}
% \vspace{-0.5em}
\end{figure}


==> figure_tex/fig_effect_tree_reduction_gpu_sddmm.tex <==
\begin{figure}[t]
\centering

\includegraphics[width=0.75\linewidth]{figure_raw/effect_tree_reduction_gpu_sddmm_rand_100K.pdf}

\caption{Effect of tree reduction on the GPU performance of dot-product attention. Tested on \texttt{rand-100K}.}
\label{fig:effect-tree-reduction-gpu-sddmm}
\end{figure}
 

==> figure_tex/fig_hybrid_partitioning_gpu.tex <==
\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{figure_raw/hybrid_partitioning_gpu.pdf}
\caption{Hybrid partitioning to make effective use of shared memory with limited capacity.}
\label{fig:hybrid-partitioning-gpu}
\end{figure}

